What to Preserve and What to Transfer: Faithful, Identity-Preserving Diffusion-based Hairstyle Transfer

Hairstyle transfer is a challenging task in the image editing field that modifies the hairstyle of a given face image while preserving its other appearance and background features. The existing hairstyle transfer approaches heavily rely on StyleGAN, which is pre-trained on cropped and aligned face images. Hence, they struggle to generalize under challenging conditions such as extreme variations of head poses or focal lengths. To address this issue, we propose a one-stage hairstyle transfer diffusion model, HairFusion, that applies to real-world scenarios. Specifically, we carefully design a hair-agnostic representation as the input of the model, where the original hair information is thoroughly eliminated. Next, we introduce a hair align cross-attention (Align-CA) to accurately align the reference hairstyle with the face image while considering the difference in their head poses. To enhance the preservation of the face image's original features, we leverage adaptive hair blending during the inference, where the output's hair regions are estimated by the cross-attention map in Align-CA and blended with non-hair areas of the face image. Our experimental results show that our method achieves state-of-the-art performance compared to the existing methods in preserving the integrity of both the transferred hairstyle and the surrounding features. The codes are available at https://github.com/cychungg/HairFusion

==> text/7_rebuttal.tex <==
\section{(KxHC, 6)}
\subsection{Review}
% 원문
"Hairstyle transfer, which modifies the hairstyle of a given face image, is a challenging task in the field of image editing due to the need to preserve fine-grained details of reference hairstyles under extreme pose variations, this paper proposes a diffusion-based image editing approach named HairFusion. It generates high-fidelity images with the reference hairstyle while preserving the surrounding features. Its main novelty lies in its hair-agnostic representation, which eliminates the hair information from the original image while preserving other regions. The pipeline also includes a cross-attention mechanism to align the reference hairstyle with the aforementioned agnostic representation. An adaptive hair blending method is also introduced to address the issue of handling occluded regions in the agnostic representation. Extensive experiments have demonstrated the effectiveness of the method.

Pros: This paper introduces the first one-stage diffusion-based hairstyle transfer framework, with three uniquely designed modules, which contributes to its novelty and originality. The pipeline is well-structured and easy to follow, with clear explanations of the proposed methods. The visualization results are also inspiring.

Cons: 
1) The paper's main motivation is not strong enough. Although it emphasizes being the first one-stage diffusion approach for hairstyle transfer, it does not clearly distinguish hairstyle transfer from other tasks, such as clothing transfer. The specific challenges that make hairstyle transfer uniquely difficult should be better articulated to justify the proposed methodology; otherwise, the method's significance may seem less convincing. 

2) In the quantitative experimental section, Table 1 shows that the SYH method is applied to the K-Hairstyle dataset but is absent from the CelebV-Text dataset, which raises curiosity without further explanation. 

3) Additionally, the ablation study indicates that even the baseline without cross-attention or adaptive blending outperforms compared methods like SYH, PbE, and Anydoor. This suggests that the compared baselines might not be state-of-the-art, which weakens the persuasiveness of the proposed method."

\subsection{Answer}
% 답변
% We truly appreciate valuable feedback. We will add all the points we discussed in the final paper.
% 1) main motivation
% 인페인팅 특성상 이미지에서 bbox로 물체를 빼고 다시 reconstruction으로 학습을 하면서 오버피팅
% 헤어에서도 결국 같은 사람의 헤어로 다른 뷰의 같은 사람을 recon
% unpaired가 아니니까 추론에서 다른 사람끼리 합성하면 두상이 안맞는 등의 어색한 부분이 생김
% 완화하는게 제일 큰 문제
% 헤어만의 유니크한 문제는 그 오버피팅을 훨씬 많이 완화해야한다는 것인데
% 유체 non rigid라서 자유도 stochasticity가 더 높음 -> spatial feature를 주입하고, face outline과 함께 align, token 단위 seg로 해결했다
% 사람과의 다양한 part와도 연관이 되어있어서 occluded part도 훨씬 복잡하고 큼, 생성하는 범위 더 넓음 (단발, 장발) 다른 다양한 신체부위 침해하는 경우 많음 -> % adaptive blending
% 소파 > 옷 > 사람얼굴 > 헤어
% We conceptualize hairstyle transfer as reference-based image inpainting.
% In common reference-based image inpainting methods such as PbE[1] and Anydoor[2], reference objects such as dolls and chairs mostly require rigid transformation to fit the source image.
% That is, the reference objects are allowed to maximally preserve their original shapes when injected into the source image.
% Similarly, in a virtual try-on, it is essential to preserve small logos and delicate patterns on the reference clothing when transferring it to the source image.

% In clothing transfer, it is essential to preserve small logos and delicate patterns on the reference clothing when transferring it to the source image.
% Therefore, it requires rigid transformation to maximally preserve their original shapes when injected into the source image.

% However, hairstyle transfer poses unique challenges due to the high variability in shape within a single hairstyle, as the hair shape strongly depends on the source features.
% When transferred to the source image, the shape of the reference hairstyle can become significantly deformed as it interacts with the face, upper body, clothing, and background, as shown in Fig. 1 in the main paper. 
% To achieve a natural fit, reference hairstyles require a more flexible transformation that allows them to blend seamlessly with the source’s original features.
% Additionally, source and reference hairstyles often differ significantly in width and length, resulting in larger occlusion regions that contain more complex structures and textures (e.g., face, clothing, background, etc.).

% reference hair or cloth를 source 에 align 시켜서 합성해야한다는 점에서 clothing transfer와 hairstyle transfer는 비슷하다.
% 하지만, clothing transfer의 경우 inpainting region이 어느 정도 정해져 있다.
% 예를 들어, 상의의 경우 팔을 포함한 상체, 하의의 경우 다리를 포함한 하체에 국한된다.
% 이에 반해, hairstyle transfer의 경우 hair의 width와 length가 헤어 별로 variability가 높기 때문에, inpainting region의 자유도가 훨씬 높다.
% 예를들어 단발의 경우 얼굴의 일부만 침범하지만, 장발의 경우 얼굴은 물론 상체의 많은 영역까지 침범이 가능하며
% 얼굴만 보더라도 앞머리나 옆머리에 따라 이마, 눈썹, 귀 등 다양한 texture를 가진 영역의 침범 여부가 결정된다. 
% 따라서 다양한 reference hair를 입히기 위해서는 source image의 상당히 넓은 영역을 potential hair region 으로 간주해야한다.
% 예를 들어 단발의 경우 source hair 로 인한 occlusion은 미미하지만, 장발 hair가 입혀질 경우를 대비해서 상체의 많은 영역까지 미리 inpainting region으로 간주하여 masking해야한다. 
% 또한 결과적으로 hair가 입혀지지 않은 영역에 대해서는 정교한 inpainting 작업이 이루어 져야 한다.
% 예를 들어 앞머리가 있는 장발을 앞머리가 단발로 바꿀 경우, 이마, 눈썹, 목, 옷, 배경 등의 다양한 영역을 결과 이미지에서 복원해 내야 한다.

1) Unique challenges of hairstyle transfer
Hairstyle transfer and clothing transfer are similar in that both require aligning the reference hair or clothing with the source image to synthesize the desired output.
However, hairstyle transfer requires a much broader range of the inpainting region than clothing transfer, making it more challenging.
For example, in clothing transfer, the inpainting region for tops is confined to the torso and arms, while the inpainting region for bottoms is restricted to the legs.
In contrast, hairstyle transfer has much more diverse inpainting regions due to the high variability in hair width and length across different hairstyles.
For instance, short hair may only affect a small portion of the face, while long hair can impact not only the face but also much of the upper body, as shown in the second column of Fig. 1 in the main paper. 
Therefore, to apply various reference hairstyles, all the potential hair regions in the source image need to be masked as an inpainting region. 
Then, in the final output, the inpainting regions that are not covered by hair need to be realistically inpainted with various textures, including the forehead, eyebrows, neck, clothing, and background.
To address this unique challenge, we carefully design a hair-agnostic representation that faithfully removes all the potential hair regions.
Also, we propose adaptive hair blending to reconstruct source features in the inpainting regions that are not covered by the reference hair.
In this way, our method can transfer a wide range of reference hairstyles including in-the-wild samples, while maximally preserving the source features.

% using hair segmentation masks, DensePose[6], and facial landmarks.
% Even within the face, the presence of bangs or sideburns determines the occlusion of various features, such as the forehead, eyebrows, and ears.

% 2) SYH CelebV 결과
2) Comparison to SYH using CelebV-Text dataset
We conduct a quantitative comparison to SYH using the CelebV-Text using the same settings as in Table 1 of the main paper as follows:
       | FID↓  |SSIM↑ | PSNR↑ | LPIPS↓
SYH    | 35.77 | 0.62 | 21.14 | 0.30
Ours   | 23.50 | 0.74 | 22.55 | 0.18
The result shows that our method achieves superior performance in all metrics.


%        | FID↓  |SSIM↑ | PSNR↑ | LPIPS↓
% SYH    | 35.77 | 0.62 | 21.14 | 0.30
% PbE    | 32.72 | 0.41 | 14.55 | 0.42
% Anydoor| 35.70 | 0.50 | 15.45 | 0.37
% Ours   | 23.50 | 0.74 | 22.55 | 0.18


% 3) ablation baseline 해명
% "일부 메트릭은 쟤네가 잘한다 
% 우리 baseline은 pbe+ controlnet
% -> controlnet으로 spatial feature를 넣어줘서 좀 좋아진거고 
% 근데 여전히 부족해서 더 개선시킨 것
% 최근 sota 베이스라인 실험까지 묶어서 서술"
3) Baseline performance in the ablation study
In the main paper, our baseline in Table 3 achieves inferior performance compared to other methods in Table 1, except for the FID score.
Our baseline (=PbE+hair encoder) may achieve a better FID score due to the enhanced hair features injection.
Since the baseline still struggles to properly align the target hair and realistically inpaint the occlusion, we improve it by adding the Align-CA and adaptive hair blending, as presented in Table 3 and Fig. 8.

% In the main paper, our baseline in Table 3 achieves inferior performance compared to other methods in Table 1 for all the metrics, except for the FID score.
% Our baseline may achieve a better FID score since it consists of PbE and an additional hair encoder that injects more detailed spatial hair features.
% However, the baseline still struggles to properly align the target hair features and realistically inpaint the occluded regions in the source, we improve its performance by adding the Align-CA and adaptive hair blending, as presented in Table 3 and Fig. 8.
% Our method also achieves superior performance when compared to the more recent state-of-the-art methods, HairFastGAN and Stable-Hair, using cropped and aligned K-Hairstyle dataset as follows:

% Method         | FID↓  |SSIM↑ | PSNR↑ | LPIPS↓
% -------------------------------------------
% HairFastGAN[4] | 19.37 | 0.52 | 17.19 | 0.36
% Stable-Hair[5] | 30.02 | 0.50 | 16.91 | 0.32
% Ours           | 15.41 | 0.55 | 19.26 | 0.30

% We conduct experiments using the same settings as in Table 2 of the main paper.
% % fid 안좋은이유 추가
% We will add the results and clarify the architecture of the baseline in Table 3 in the final paper.

% SYH     22.84  0.62  18.41
% PbE     13 26  0 59  19 26  0 29
% Anydoor 19 00  0 63  18 78  0 27
% Ours    15 43  0 58  18 09  0 30



%%%%%%%%%%%%%%%%%%%%%%% final %%%%%%%%%%%%%%%%%%%%%%%% (글자수 맞춤)
We appreciate valuable feedback. We will add all the points we discussed in the final paper.

1) Motivation

Hairstyle transfer and clothing transfer are similar in that both require aligning the reference hair or clothing with the source image to synthesize the desired output.
However, hairstyle transfer requires a much broader range of the inpainting region than clothing transfer, making it more challenging.
For example, in clothing transfer, the inpainting region for tops is confined to the torso and arms, while the inpainting region for bottoms is restricted to the legs.
In contrast, hairstyle transfer has much more diverse inpainting regions due to the high variability in hair width and length across different hairstyles.
For instance, short hair may only affect a small portion of the face, while long hair can impact not only the face but also much of the upper body, as shown in the second column of Fig. 1 in the main paper.
Therefore, to apply various reference hairstyles, all the potential hair regions in the source image need to be masked as an inpainting region.
In the final output, the inpainting regions not covered by hair need to be realistically inpainted with various textures, including the forehead, eyebrows, neck, clothing, and background.
To address this unique challenge, we carefully design a hair-agnostic representation that faithfully removes all the potential hair regions.
We also propose adaptive hair blending to reconstruct the removed source features in the inpainting regions that are not covered by the reference hair.
In this way, our method can transfer a wide range of reference hairstyles including in-the-wild samples, while maximally preserving the source features.

2) SYH comparison

We conduct a quantitative comparison to SYH using the CelebV-Text using the same settings as in Table 1 of the main paper. The result shows ours achieves superior performance in all metrics:
|| FID↓|SSIM↑| PSNR↑|LPIPS↓|
|-|-|-|-|-|
|SYH|35.77|0.62|21.14|0.30
|Ours|**23.50**|**0.74**|**22.55**|**0.18**

3) Baseline in the ablation

In the main paper, our baseline in Table 3 achieves inferior results compared to other methods in Table 1, except for FID score.
Our baseline(=PbE+hair encoder) may achieve a better FID due to the enhanced hair features injection.
Since the baseline still struggles to properly align the target hair and inpaint the occlusion, we improve it by adding the Align-CA and adaptive hair blending, as shown in Table 3 and Fig. 8.



\section{(qC2M, 4)}
\subsection{Review}
% 원문
The work lacks innovation. Hair-agnostic representation has been used in the VITON field for a long time, and blending is common in both virtual try-on and diffusion-based methods. Additionally, the simple mask design is insufficient to claim a novel contribution. The limited number of comparison methods fail to demonstrate the advancement of the proposed approach. There are also concerns about fairness in the comparisons, and the visualizations present numerous issues, particularly regarding the preservation of irrelevant attributes, especially in terms of clothing.

Pros 1.Compared to StyleGAN methods, the visual effects for multi-colored hairstyles are superior to those based on StyleGAN. 2.It effectively addresses the issue of in-the-wild samples. 3.This diffusion-based pipeline can achieve hairstyle transfer in a single step.

Cons 1.Agnostic representation has been used in the VITON field for some time[1], and the simple mask design is insufficient to qualify as an innovation. 

2.Blending techniques have been widely employed in virtual try-on[4], including various inpainting-related method[2]. 

3.The lack of comparisons is notable; Barbershop also demonstrates strong hairstyle and face alignment capabilities, alongside recent works like StyleGAN-Salon[5], HairFastGAN[7], and Stable-Hair[6], which claims to be the first diffusion-based method for hair transfer. Your method shows noticeable gaps in color fidelity and hairstyle accuracy compared to Stable-Hair. 

4.Regarding the visual results, significant clothing changes are apparent in the first row of Fig. 1, columns one to three, and the second row, column two. In Fig. 4(b), the hair region outside the inpainting area lacks control, leading to many ambiguous yellow hairs. 

5.A minor issue in Fig. 4(a): the face in the lower section is not obscured, which may raise ethical concerns; K-hairstyle may have overlooked this in facial information removal. 

6.The comparison is unfair; StyleGAN methods are trained on datasets like CelebA and FFHQ, where most previous hairstyle editing comparisons have occurred. The removal of facial information in the K-hairstyle dataset could skew comparisons. StyleGAN’s latent space, particularly the FS space, retains facial features effectively, so comparing against StyleGAN methods using CelebA or FFHQ would be more convincing.

[1] [2103.16874] VITON-HD: High-Resolution Virtual Try-On via Misalignment-Aware Normalization (arxiv.org) [2] [2403.06976] BrushNet: A Plug-and-Play Image Inpainting Model with Decomposed Dual-Branch Diffusion (arxiv.org) [3] [2312.01725] StableVITON: Learning Semantic Correspondence with Latent Diffusion Model for Virtual Try-On (arxiv.org) [4] [2407.15886] CatVTON: Concatenation Is All You Need for Virtual Try-On with Diffusion Models (arxiv.org) [5] [2304.02744] StyleGAN Salon: Multi-View Latent Optimization for Pose-Invariant Hairstyle Transfer (arxiv.org) [6] [2407.14078] Stable-Hair: Real-World Hair Transfer via Diffusion Model (arxiv.org) [7] [2404.01094] HairFastGAN: Realistic and Robust Hair Transfer with a Fast Encoder-Based Approach (arxiv.org)

\subsection{Answer}
% 답변
% 1. agnostic representation 
% "VITON-HD에 나와있는것은 body이고 우리는 얼굴 주변이라서 포인트가 다르다
% viton은 skeleton이라는 좋은 그게 있는데 우리는 없어서 head 포인트와 얼굴 윤곽을 잡기위해 이런이런 방식을 써서 했다 어필"	"헤어 쪽에서는 처음이 맞음
% VITON HD에서도 처음으로 제안을했고 이건 그 뒤로도 많이 쓰이고 powerful 했으니 우리도 의미 있다고 볼 수 있다.
1) Agnostic representation
While the inpainting region in VITON is limited to the torso and arms or legs, hairstyle transfer has a much broader range of the inpainting regions due to variable hair width and length across different hairstyles, making it more challenging.
For instance, short hair may only affect a small portion of the face, while long hair can impact not only the face but also much of the upper body, as shown in Fig. 1 in the main paper. 
Therefore, to apply various reference hairstyles, we carefully design a hair-agnostic representation that faithfully removes all the potential hair regions using hair masks, DensePose, and facial landmarks.
As the agnostic representation introduced by VITON-HD has become widely used in the VITON field, our hair-agnostic representation offers a meaningful impact on the advancements in hairstyle transfer.


% 2. blending
% "BrushNet, CatVTON 살펴보고 차별점 어필 (헤어 관련해서)
% -> BrushNet은 이미 있는 mask로 blurry blending 우리는 align-ca에서 생성될 영역을 미리 알아낸다는 점이 중요
% CAT은 blending 없음 
% 헤어만의 문제를 어필하고 연결지어서"
2) Blending
The existing blending techniques in the VITON field or BrushNet simply utilize the input inpainting mask as its blending mask.
However, since all the potential hair regions are removed in the inpainting mask, using the input inpainting mask as a blending mask is insufficient to maximally preserve source features.
Therefore, our adaptive hair blending generates a novel adaptive blending mask by estimating the output's hair region using cross-attention maps in Align-CA.
In this way, HairFusion can effectively apply various reference hairstyles while maximizing the maintenance of the source features.


% 3. lack of comparison
% stylegan 웍의 대표로 style your hair 과 hair clip v2를 진행 했던 것인데,  the most recent stylegan-based 모델인 HairfastGAN 이랑  concurrent 지만 stable hair까지 같이 해봤다.
% 시간상 pretrained로 해봤다 align이미지로 우리 main table이랑 똑같이 했을때 여전히 우리보다 못한다 
% hairfast gan은 aligned 이미지를 base로 한 stylegan을 사용해서 style your hair처럼 unaligned 이미지들에 대해서는 못할 가능성이 높다.
% unaligned로 학습을 해서 최대한 final paper에 비교실험을 해보겠다
% stable hair의 경우 unalgined 이미지들 paired 데이터를 구축하고, bald 이미지 생성 모델을 unaligned이미지에 대해 새로 학습해본다면 더 좋은 성능을 낼 수 있을 것 같은데, 
% 그런 paired data 구축이나 bald 변환 모델 없이 end to end diffusion-based로는 우리가 처음이고 cost 측면에서 더 경쟁력을 가진다
3) Lack of comparison
Our method achieves superior performance compared to the most recent StyleGAN-based method, HairFastGAN, and concurrent diffusion-based method, Stable-Hair:
        |FID|SSIM|PSNR|LPIPS
HairFastGAN|19.37|0.52|17.19|0.36
Stable-Hair |30.02|0.50|16.91|0.32
Ours      |15.41|0.55|19.26|0.30
In our experiments, Stable-Hair might achieve an inferior FID score due to the artifacts generated in bald proxy images.
Due to the time limit, we conduct experiments using the pretrained models from official codes and aligned images as in Table 2 of the main paper.
We will conduct additional experiments with unaligned images and add the results to the final paper.

% 4. visual result
4) Visual result
As presented in Fig. 4, 5, and 6 in the main paper, ours produces superior visual results compared to other methods, effectively preserving reference hair and source features.
% blending의 경우에는 cross attention 이 영역을 잡은 만큼 유지가 된다 이 threshold를 조절해서 더 나은 결과를 도출할 수도 있다

% 6. unfair comparison
% "우선 removal이 안된 상태에서 하는거고 직접 stylegan을 학습시켜서 돌린거라 fair한 비교이다
% 우리 메소드는 multi view dataset이 필요해서 celebA랑 FFHQ로는 불가능해서 우리가 직접 multiview로 학습시킨 모델을 가지고 비교한 결과가 여기있고 우리가 성능이 더 좋았다"
% The comparison is unfair; StyleGAN methods are trained on datasets like CelebA and FFHQ, where most previous hairstyle editing comparisons have occurred. The removal of facial information in the K-hairstyle dataset could skew comparisons. StyleGAN’s latent space, particularly the FS space, retains facial features effectively, so comparing against StyleGAN methods using CelebA or FFHQ would be more convincing.
5) Unfair comparison
The faces of K-hairstyle images used in the experiments have not been removed. 
The faces are removed only for the visualization due to the privacy issue.
Also, for a fair comparison, we retrain the StyleGAN using K-hairstyle and CelebV-Text for the experiments in Table 1.

%%%%%%%%%%%%%%%%%%%%%%% final %%%%%%%%%%%%%%%%%%%%%%%% (글자수 맞춤)
We appreciate valuable feedback. We will add all the discussed points in the final paper.

1) Agnostic

While the inpainting region in VITON  is limited to the torso, arms, or legs, hairstyle transfer has a broader range of inpainting regions due to variable hair width and length across different hairstyles, making it more challenging.
For instance, short hair may only affect the face, while long hair can impact both the face and the upper body, as in Fig. 1 in the main paper.
Therefore, to apply various hairstyles, we carefully design a hair-agnostic representation that faithfully removes all the potential hair regions using hair masks, DensePose, and facial landmarks.
As the agnostic representation introduced by VITON-HD has been widely used in VITON, our hair-agnostic representation offers a meaningful contribution to hairstyle transfer.

2) Blending

The existing blending techniques in VITON or BrushNet utilize the inpainting mask as a blending mask.
However, since all the potential hair regions are removed in our inpainting mask, using it as a blending mask is insufficient to maximally preserve source features.
Therefore, our adaptive hair blending generates a novel adaptive blending mask by estimating output's hair region using cross-attention maps in Align-CA, further enhancing maintenance of source features.

3) Lack of comparison

Ours achieves superior performance compared to the most recent StyleGAN-based method, HairFastGAN (1), and a concurrent diffusion-based method, Stable-Hair (2):

||FID↓|SSIM↑| PSNR↑|LPIPS↓|
|-|-|-|-|-
|(1)|19.37|0.52|17.19| 0.36
|(2)|30.02 |0.50|16.91|0.32
|Ours|**15.41**|**0.55**|**19.26**|**0.30**

In our experiment, Stable-Hair (2) may achieve inferior FID due to artifacts generated in bald proxy images.
Due to time limit, we use pretrained models from official codes and aligned images as in Table 2 of the main paper. We will conduct experiments with unaligned images and add them to the final paper.

4) Visual result and face removal

As in Fig. 4, 5, and 6 in the main paper, ours produces superior results compared to other methods, effectively preserving both reference hair and source features. We will remove the face of the K-hairstyle images in the final paper.

5) Unfair comparison

The faces of K-hairstyle used in the experiments have not been removed but removed only in visualization for privacy. 
Also, for a fair comparison, we retrain the StyleGAN using K-hairstyle and CelebV-Text for the experiment in Table 1.




\section{(QFo4, 6)}
\subsection{Review}
% 원문
The paper proposes HairFusion, a diffusion-based model for hairstyle transfer.

The contributions are;

Hair-Agnostic Representation: Removes the hair region from the source image using segmentation masks, helping the model focus on hair alignment.
Align Cross-Attention (Align-CA): Uses cross-attention between face and hair features, guided by face outline images, to align the reference hairstyle with the source face, addressing pose and shape differences.
Adaptive Hair Blending: Blends the generated hair with non-hair areas using attention-based masks, aiming to preserve facial details and minimize blending errors.
Strength:

Align-CA and attention based blending is innovative for hairstyle transfer and clearly improves results, as shown in Figure 8
The paper is well written and easy to understand

Weakness:

1) Missing comparison with recent works like StyleGAN-Salon, which also claims to handle pose disparity. There is also no user study, which is crucial for fair comparison in this subjective setting.

2) The overall pipeline is complex with several hand-engineered parts, such as manually removing hair regions in the hair-agnostic representation. It also requires face outline inputs alongside source and target images, adding extra complexity and dependency on other methods.

3) The results for in-the-wild images in Figure 1 appear somewhat unnatural to me, and even when poses are similar, there are noticeable differences between the result hairstyle and the reference hairstyle.
Questions:

2)에 포함 Where does the face outline come from? I assume that during testing, it should be extracted using the same method used during training?

Overall, I think the contributions of the paper are quite valuable, especially as the first to apply diffusion models to hairstyle transfer. However, I do have some concerns about the results, especially with the missing comparison to the previous state-of-the-art methods. Despite these concerns, however, I lean towards a borderline accept.


\subsection{Answer}
% 답변
% 1) comparison to baselines and user study
% stylegan 웍의 대표로 style your hair 과 hair clip v2를 진행 했던 것인데,  the most recent stylegan-based 모델인 HairfastGAN 이랑  concurrent 지만 stable hair까지 같이 해봤다.
% 시간상 pretrained로 해봤다 align이미지로 우리 main table이랑 똑같이 했을때 여전히 우리보다 못한다 
% hairfast gan은 aligned 이미지를 base로 한 stylegan을 사용해서 style your hair처럼 unaligned 이미지들에 대해서는 못할 가능성이 높다.
% unaligned로 학습을 해서 최대한 final paper에 비교실험을 해보겠다
% stable hair의 경우 unalgined 이미지들 paired 데이터를 구축하고, bald 이미지 생성 모델을 unaligned이미지에 대해 새로 학습해본다면 더 좋은 성능을 낼 수 있을 것 같은데, 
% 그런 paired data 구축이나 bald 변환 모델 없이 end to end diffusion-based로는 우리가 처음이고 cost 측면에서 더 경쟁력을 가진다
% User study 는 시간상 못했는데 final paper에 꼭 싣도록 하겠다
1) Lack of comparison and user study
We conduct a comparison to the most recent StyleGAN-based method, HairFastGAN, and the concurrent diffusion-based method, Stable-Hair, as follows:
                  |FID|SSIM|PSNR|LPIPS
HairFastGAN|19.37|0.52|17.19|0.36
Stable-Hair |30.02|0.50|16.91|0.32
Ours         |15.41|0.55|19.26|0.30
Ours achieves superior performance over the others.
Stable-Hair may achieve inferior FID due to artifacts generated in bald proxy images.
Due to the time limit, we conduct experiments using pretrained models and aligned images as in Table 2 of the main paper.
We will conduct additional experiments with unaligned images and add them to the final paper.

% 2) agnostic과 face outline hand engineered
% "이게 필요한 이유 agnostic의 중요성, 어려움 어필, 그리고 그리 복잡하지 않다.
% face outline image는 facial landmark로 부터 쉽게 뽑아낼 수 있고 방법 설명, 뽑는 코드를 officially 제공할 예정이다."	헤어만의 차별점 어필해서 agnostic 중요성 언급
2) Hand-engineered agnostic representation and face outline image
Hairstyle transfer has diverse inpainting regions due to the high variability in hair width and length across different hairstyles.
For instance, short hair may only affect a small portion of the face, while long hair can impact not only the face but also much of the upper body, as shown in the second column of Fig. 1 in the main paper. 
Therefore, to apply various reference hairstyles, all the potential hair regions in the source image need to be masked as an inpainting region. 
To address this issue, we carefully design a hair-agnostic representation that faithfully removes all the potential hair regions using hair segmentation masks, DensePose, and facial landmarks.
We will clarify the process of generating the agnostic representation in the final paper.
Also, the face outline images are obtained by simply drawing lines between the facial landmarks extracted by a pretrained detector.
The source code for extracting face outline images will be made publicly available following the publication of this paper.


% 3) visual results
% "그래도 다른 메소드에 비해 월등한 성능이다
% blending의 경우에는 cross attention 이 영역을 잡은 만큼 유지가 된다 이 threshold를 조절해서 더 나은 결과를 도출할 수도 있다
% 다양한 포즈에 대한 결과는 supple에서 더 볼 수 있다 최종 페이퍼에 더 다양한 결과를 추가하겠다
3) Visual result
As presented in Fig. 4, 5, and 6 in the main paper, ours produces superior visual results compared to other methods, effectively preserving both reference hair and source features.
Results with more diverse head poses are in the supplementary.

%%%%%%%%%%%%%%%%%%%%%%% final %%%%%%%%%%%%%%%%%%%%%%%% (글자수 맞춤)
We appreciate valuable feedback. We will add all the discussed points in the final paper.

1) Lack of comparison and user study

We conduct a comparison to (1)HairFastGAN, a more recent StyleGAN-based method than StyleGAN-Salon, and (2)Stable-Hair, a concurrent diffusion-based method:
|| FID↓|SSIM↑| PSNR↑|LPIPS↓|
|-|-|-|-|-|
|(1)|19.37|0.52|17.19| 0.36
|(2)|30.02 |0.50|16.91|0.32
|Ours|**15.41**|**0.55**|**19.26**|**0.30**

Ours achieves superior performance over the others.
In our experiment, (2)Stable-Hair may achieve inferior FID due to artifacts generated in bald proxy images.
Due to the time limit, we conduct experiments using pretrained models from official codes and aligned images as in Table 2 of the main paper.
We will conduct additional experiments including user study with unaligned images and add them to the final paper.

2) Hand-engineered agnostic representation, face outline image

Hairstyle transfer has diverse inpainting regions due to the high variability in hair width and length across different hairstyles.
For instance, short hair may only affect a small portion of the face, while long hair can impact not only the face but also much of the upper body, as shown in the second column of Fig. 1 in the main paper. 
Therefore, to apply various reference hairstyles, all the potential hair regions in the source image need to be masked as an inpainting region. 
To address this issue, we carefully design a hair-agnostic representation that faithfully removes all the potential hair regions using hair segmentation masks, DensePose, and facial landmarks extracted from external models.
Although this process might seem complex, it allows our method to transfer diverse reference hairstyles while preserving the source features.
Constructing a hairstyle transfer model without relying on external models could be one promising future research direction.

Additionally, the face outline images are obtained by simply drawing lines between the facial landmarks extracted by a pretrained detector.
The existing hairstyle transfer approaches also leverage similar preprocessing steps.
The source codes for extracting face outline images will be made publicly available following the publication of this paper.

3) Visual result

As presented in Fig. 4, 5, and 6 in the main paper, ours produces superior visual results compared to other methods, effectively preserving both reference hair and source features.
Results with more diverse head poses are in the supplementary.



\section{(75Jy, 8)}
\subsection{Review}
% 원문
This paper proposes a novel diffusion-based method for hairstyle transfer and shows excellent experimental results.

Strengths:

The proposed method is novel and well-motivated. The paper is clearly written.
Quantitative and visual results outperform state-of-the-art methods.
The experiments are comprehensive for evaluating effectiveness.
It is interesting and inspirational that the proposed Align-CA can align features with different poses.
Weaknesses:

Note that any weaknesses related to the lack of experiments require only a discussion as part of the rebuttal and not new experimental result.

1) Missing reference:
Chang et al. Hairnerf: Geometry-aware image synthesis for hairstyle transfer
Nikolaev et al. HairFastGAN: Realistic and Robust Hair Transfer with a Fast Encoder-Based Approach

2) I feel like the limitations shown in the paper are not the key. The authors are supposed to add some failure cases and discuss about limitations of the differences between the synthesized hairstyle and the one in the reference image (I can see minor differences like bang thickness, and appearance in Fig. 2 of the supp.)

3) The used hairstyles are somehow simple (maybe in the training dataset distribution). I am curious about the edge of the hair feature extractor: will it work well on complex Afro hair or even cartoon images?


\subsection{Answer}
% 답변
% 1) missing reference 
% 추가하겠다 hairfastGAN은 비교까지 해봤고 우리가 더 좋은 성능을 보였다 이 결과도 main 에 싣겠다
1) Missing reference
Thank you for pointing it out.
We will add the references to the final paper.
We also conduct an additional comparison to the most recent StyleGAN-based method, HairFastGAN, and the concurrent diffusion-based method, Stable-Hair, as follows:
                  |FID|SSIM|PSNR|LPIPS
HairFastGAN|19.37|0.52|17.19|0.36
Stable-Hair |30.02|0.50|16.91|0.32
Ours         |15.41|0.55|19.26|0.30
Ours achieves superior performance over the others.
Stable-Hair may achieve inferior FID due to artifacts generated in bald proxy images.
Due to the time limit, we conduct experiments using pretrained models and aligned images as in Table 2 of the main paper.
We will conduct additional experiments with unaligned images and add them to the final paper.


% 2) limitation
% limitation을 좀 더 설명 (external model에 대한 의존, 디테일한 영역들에 대한 복원 문제), 더 명확하게 보이는 사례를 추가하겠다. 	"(인페인팅 기술이라서 hyperparameter에 따라) 좀 달라지는 헤어외의 영역이 있다 
% 이런것도 중요한 limitation일 수 있다, 개선될 수 있다 (새로운 approach 언급 x)"
2) Limitation
High dependence on external models, such as facial landmark detectors and face parsing models, can limit the overall performance of the model.
Errors in the extraction of facial landmarks or parsing maps can introduce undesirable artifacts into the results. One way to address this is by either improving the accuracy of these external models or by integrating facial landmark detection and face parsing directly into our model, creating a self-sufficient solution.

Additionally, reconstructing detailed features near the hairline can be challenging, often leading to unnatural results, as noted by other reviewers. 
To mitigate this, controlling hyperparameters in adaptive hair blending can help improve the preservation of source features, making the results more natural.
We will include additional results in the final paper that show the limitations of our method more clearly.



% 3) edge case hairstyles
% figure 1에 이런이런 독특한 hairstyle도 잘한다 말해준 complex Afro나 cartoon image도 diffusion의 힘으로 잘될 것 같은데 실험해서 final paper에 edge case에 대해서도 추가해보겠다
3) Edge cases
As shown in Fig. 1 of the main paper, our method effectively transfers a variety of hairstyles, including those with multiple colors or complex curls. 
Additional results with more diverse hairstyles are provided in the supplementary materials. 
In the final paper, we will include even more challenging hairstyles, such as Afro and cartoon styles, to further demonstrate the versatility of our approach.


%%%%%%%%%%%%%%%%%%%%%%% final %%%%%%%%%%%%%%%%%%%%%%%% (글자수 맞춤)
We appreciate valuable feedback. We will add all the points we discussed in the final paper.

1) Missing reference

Thank you for pointing it out.
We will add the references to the final paper.
We also conduct an additional comparison to the most recent StyleGAN-based method, HairFastGAN, and the concurrent diffusion-based method, Stable-Hair, as follows:
|| FID↓|SSIM↑| PSNR↑|LPIPS↓|
|-|-|-|-|-|
|HairFastGAN|19.37|0.52|17.19| 0.36
|Stable-Hair|30.02 |0.50|16.91|0.32
|Ours|**15.41**|**0.55**|**19.26**|**0.30**

Ours achieves superior performance over the others.
In our experiments, Stable-Hair may achieve inferior FID due to artifacts generated in bald proxy images.
Due to the time limit, we conduct experiments using pretrained models from the official codes and aligned images as in Table 2 of the main paper.
We will conduct additional experiments with unaligned images and add them to the final paper.
We will also add Hairnerf as related work to the final paper.

2) Limitation

High dependence on external models, such as facial landmark detectors and face parsing models, can limit the overall performance of the model.
Errors in the extraction of facial landmarks or parsing maps can introduce undesirable artifacts into the results. 
One way to address this is by either improving the accuracy of these external models or by integrating facial landmark detection and face parsing directly into our model, creating a self-sufficient solution.
In addition, reconstructing detailed features near the hairline can be challenging, often leading to unnatural results, as noted by other reviewers. 
To mitigate this, controlling hyperparameters in blending mask generation of adaptive hair blending can help improve the preservation of source features, making the results more natural.
Reducing reliance on the external hair segmentation model, or improving its accuracy, can also be a feasible solution.
We will include additional results in the final paper that show the limitations of our method more clearly.

3) Edge cases

As shown in Fig. 1 of the main paper, our method effectively transfers a variety of hairstyles, including those with multiple colors or complex curls. 
Additional results with more diverse hairstyles are provided in the supplementary materials. 
In the final paper, we will include even more challenging hairstyles, such as Afro and cartoon styles, to further demonstrate the versatility of our approach.

==> text/table/ablation_old.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc}
\hline
      & Ours           & w/o blending & w/o landmark & w/o HACA \\ \hline
FID$\downarrow$   & \textbf{10.82} & 15.59        & 19.35        & 15.43    \\ \hline
SSIM$\uparrow$  & \textbf{0.70}  & 0.62         & 0.59         & 0.58     \\ 
PSNR$\uparrow$  & \textbf{21.15} & 19.33        & 17.46        & 18.09    \\ 
LPIPS$\downarrow$ &  \textbf{0.18} & 0.27        & 0.30        & 0.30     \\ \hline
\end{tabular}
}
\caption{Ablation Study.} 
\label{Tab:ablation} 
\end{table}
